ProPanDL: A Modular Architecture for Uncertainty-Aware Panoptic Segmentation

We introduce ProPanDL, a family of networks capable of uncertainty-aware panoptic segmentation. Unlike existing segmentation methods, ProPanDL is capable of estimating full probability distributions for both the semantic and spatial aspects of panoptic segmentation. We implement and evaluate ProPanDL variants capable of estimating both parametric (Variance Network) and parameter-free (SampleNet) distributions quantifying pixel-wise spatial uncertainty. We couple these approaches with two methods (Temperature Scaling and Evidential Deep Learning) for semantic uncertainty estimation. To evaluate the uncertainty-aware panoptic segmentation task, we address limitations with existing approaches by proposing new metrics that enable separate evaluation of spatial and semantic uncertainty. We additionally propose the use of the energy score, a proper scoring rule, for more robust evaluation of spatial output distributions. Using these metrics, we conduct an extensive evaluation of ProPanDL variants. Our results demonstrate that ProPanDL is capable of estimating well-calibrated and meaningful output distributions while still retaining strong performance on the base panoptic segmentation task.

==> content/discussion.tex <==
\section{Future Work}

In this section, we identify several interesting directions in which this research could be extended.

\subsubsection{Tracking} Extension of panoptic segmentation to image sequences has been proposed and is variously known as Multi-Object Panoptic Tracking (MOPT) \cite{hurtado2020mopt} or Segmenting and Tracking Every Pixel (STEP) \cite{weber2021step}. This task requires panoptic segmentation for every image, but also requires assigned instance IDs to remain consistent across multiple frames. Estimating pixel-wise uncertainties and fusing these uncertainties across multiple frames may allow for improved data association and stronger tracking performance.

\subsubsection{Domain Adaptation} Uncertainty-guided domain adaptation has been successfully applied in classification \cite{liang2019exploring} and object detection \cite{guan2021uncertainty}, but to our knowledge has not been explored for semantic or panoptic segmentation.

\subsubsection{SampleNet} As previously stated, memory requirements constrained our maximum number of SampleNet samples to $M=10$. The original authors noted that calculating the energy score loss over sample mini-batches rather than the full input greatly decreases memory consumption while still maintaining strong performance \cite{harakeh2022estimating}. Taking this approach would allow for more extensive experimentation on the impact of increasing the number of samples, as 10 may not be sufficient to fully describe the offset distributions for all pixels. In addition, we did not explore the use of optimal transport regularization employed in the original paper, which was able to improve the quality of predicted distributions in several settings.

